Efficient Visual Computing with Camera RAW Snapshots

Conventional cameras capture image irradiance on a sensor and convert it to RGB images using an image signal processor (ISP). The images can then be used for photography or visual computing tasks in a variety of applications, such as public safety surveillance and autonomous driving. One can argue that since RAW images contain all the captured information, the conversion of RAW to RGB using an ISP is not necessary for visual computing. In this paper, we propose a novel $\rho$-Vision framework to perform high-level semantic understanding and low-level compression using RAW images without the ISP subsystem used for decades. Considering the scarcity of available RAW image datasets, we first develop an unpaired CycleR2R network based on unsupervised CycleGAN to train modular unrolled ISP and inverse ISP (invISP) models using unpaired RAW and RGB images. We can then flexibly generate simulated RAW images (simRAW) using any existing RGB image dataset and finetune different models originally trained for the RGB domain to process real-world camera RAW images. We demonstrate object detection and image compression capabilities in RAW-domain using RAW-domain YOLOv3 and RAW image compressor (RIC) on snapshots from various cameras. Quantitative results reveal that RAW-domain task inference provides better detection accuracy and compression compared to RGB-domain processing. Furthermore, the proposed \r{ho}-Vision generalizes across various camera sensors and different task-specific models. Additional advantages of the proposed $\rho$-Vision that eliminates the ISP are the potential reductions in computations and processing times.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[1]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sections/Abstract.tex <==


Conventional cameras capture image irradiance on a sensor and convert it to RGB images using an image signal processor (ISP). The images can then be used for photography or visual computing tasks in a variety of applications such as public safety surveillance and autonomous driving.  One can argue that since RAW image sensor contain all the captured information, the conversion of RAW to RGB using an ISP is not necessary for visual computing. In this paper, we propose a novel $\rho$-Vision framework to perform high-level semantic understanding and low-level compression using RAW images without the ISP subsystem used for decades.
%
Considering the scarcity of available RAW image datasets, we first develop an unpaired CycleR2R network based on unsupervised CycleGAN to train  modular unrolled ISP and inverse ISP (invISP) models using unpaired RAW and RGB images. We can then flexibly generate simulated RAW images (simRAW) using any existing RGB image dataset  and finetune different models originally trained for the RGB domain to process real-world camera RAW images. We demonstrate object detection and image compression capabilities in RAW-domain using RAW-domain YOLOv3 and RAW image compressor (RIC) on snapshots from various cameras.
%
Quantitative results reveal that RAW-domain task inference provides better detection accuracy and compression compared to RGB-domain processing.  Furthermore, the proposed $\rho$-Vision generalizes across various camera sensors and different task-specific models. Additional advantages of the proposed $\rho$-Vision that eliminates the ISP are the potential reductions in computations and processing times.  
   
   

\Salnote{I like $\rho$-Vision as a title, but be aware that it will be a pain to write it in ascii and it will be difficult to search for this paper. Consider changing to RAW-Vision} 


\if 0 
%\xzhang{Recent decades have witnessed the great success of computer vision, which endows the machines with the ability to “see” and explore the world. However, most of the existing computer vision tasks are based on the RGB domain and suffer from low efficiency by incurring substantial redundant computations with the embedded Image Signal Processor (ISP), such as RAW-to-RGB conversion, repetitive encoding and decoding. To cope with the challenges, we propose a novel framework, called \sys, to perform high-level semantic understanding and low-level compression directly on the raw image sensor data, which can improve the system efficiency significantly by eliminating the redundant ISP and involved computations in conventional cameras. Specifically, we first design a modular unrolling augmented Unpaired CycleR2R (Cycle RGB to RAW) model to generate realistic RAW images from abundant RGB datasets with high robustness and interpretability, which can overcome the scarcity of available dataset of RAW images. Next, we verify that effective computer vision can be achieved directly on RAW images by finetuning the state-of-the-art object detection and image compression models in RAW-domain with the generated RAE images. Quantitative results not only reveal the superior efficiency of \sys to that of traditional RGB-domain counterparts in terms of object detection accuracy  and  compression performance, but also report the unprecedented generalization of \sys across diverse camera sensors and different task-oriented models.}
Visual cameras are vastly devised to capture instantaneous snapshots using RGB images for scene understanding and action execution in applications like public safety surveillance and autonomous driving.  {As the physical radiance of a scene is  well captured by the imaging sensor raw data (RAW), it is arguable why existing commodity cameras still embed the Image Signal Processor (ISP) to transform the RAW image to human-perceivable RGB format for visual computing.}
%
%Apparently, the processing using RGB images, a.k.a., RGB-Vision, is resource-intensive, as the embedded Image Signal Processor (ISP) in commodity cameras  involves redundant computations. %, e.g., RAW-to-RGB conversion, repetitive encoding and decoding, etc. \Salnote{Can we give specific number? avoid using e.g., and etc. in the text}
%
% , especially for the network bandwidth and computation resources .
%, which hinders its widely adoption in practice. 
{This paper proposes a novel $\rho$-Vision paradigm, of which high-level semantic understanding and low-level compression are directly executed using RAW images without requiring the ISP subsystem used for decades.
%, which eliminates the ISP subsystem placed in conventional cameras for decades.%to directly perform high-level content understanding and low-level semantic coding upon the imaging sensor Bayer data, e.g., camera RAW snapshot, by which we completely removed  the Image Signal Processor (ISP) to avoid unnecessary computations, e.g., RAW-to-RGB conversion, repetitive encoding and decoding, and improve the networking efficiency by delivering compressed semantic objects rather the entire scene.
   }
   %{ ~$\rho$-Vision is motivated by the fact that significant redundancy is presented when analysing the RGB images for analytics in existing ISP equipped cameras, where unnecessary computations, e.g., RAW-to-RGB conversion, repetitive encoding and decoding, are inevitable. 
    %}  
    %This work first identified significant redundancy by using RGB images, and developed the $\rho$-Vision to directly perform high-level content understanding and low-level semantic coding upon the imaging sensor Bayer data, e.g., camera RAW snapshot, by which we completely removed  the Image Signal Processor (ISP) to avoid unnecessary computations, e.g., RAW-to-RGB conversion, repetitive encoding and decoding, and improve the networking efficiency by delivering compressed semantic objects rather the entire scene.  
   With this aim,  considering the scarcity of available RAW image datasets,  we first develop an Unpaired CycleR2R that leverages the unsupervised CycleGAN framework to train  modular unrolled ISP and inverse ISP (invISP) models using unpaired RAW and RGB samples, with which   
   %We suggest the modular unrolling to model functions in ISP/invISP  which not only ensures the model robustness and interpretability \maz{but also massively reduces the number of samples for training.} 
   we can flexibly generate abundant RAW images (a.k.a., simRAW) using any existing RGB image dataset, and these simRAW samples can be used to finetune prevalent neural models originally developed in the RGB domain to directly process real-life camera RAW samples for task execution. Both object detection and image compression are exemplified in the RAW domain by executing RAW-domain YOLOv3 and RIC (RAW Image Compressor) on RAW snapshots from various cameras. 
   Quantitative results not only reveal the superior efficiency of RAW-domain task inference to that of traditional RGB-domain counterparts, e.g., significant improvement of detection accuracy  and  compression performance but also report unprecedented generalization of the proposed $\rho$-Vision across various camera sensors and different task-oriented models.    Apparently, an additional takeaway of the proposed $\rho$-Vision is the elimination of the ISP which potentially saves computations and reduces the processing delay. 
%   \zhihao{1. robustness, remove}
%   \zhihao{2. number of samples, similar sentences}
   
   
%   \Salnote{The abstract needs major changes. Impact and contributions are not clear.}

  % and reduce the bit rate by \SI{95}{\percent} when comparing to the most popular JPEG coder at the same quality.
    %The dataset and pretrained models will be made publicly accessible for reproducible research after publication. 
   
   
   %devise an unsupervised generative adversarial network (GAN) model  to generate  RAW images from existing RGB datasets, which \xzhang{can ***}. With the generated RAW images, 
   
   %we design a Convolutional Neural Network (CNN) empowered object detection model in the RAW-domain, which can achieve competitive efficiency to those prevailing conventional models in the RGB-domain. Besides, we further propose a supervised variational autoencoder (VAE) to compress the RAW images, which can significantly improve the  efficiency of network sharing or storage.
    
    %integrated semantic cues extracted from preceding  task, e.g., segmentation task, to enable the image compression of arbitrary-shaped objects in RAW domain, e.g., $\rho$-OBIC, via a supervised variational autoencoder (VAE). 
    
  %To verify the effectiveness of $\rho$-Vision, extensive 
  %The proposed $\rho$-Vision is then evaluated using thousands of RAW images collected from a variety of image sensors used in commodity cameras.
   % We later collected and labelled seoeral thousands of RAW images using a variety of image sensors equipped in real-life cameras.  
    %Extensive field studies demonstrate the competitive efficiency and generalization of our proposed $\rho$-Vision to the state-of-the-art approaches in the RGB-domain. 
    %Besides, $\rho$-Vision can eliminate latency incurred by ISP, and reduce the bit rate by \SI{95}{\percent} when comparing to the most popular JPEG coder at the same quality.
   % The dataset and relevant materials will be made publicly accessible for reproducible research after publication. 
    
   % Besides, RAW-domain object detection eliminates the ISP latency which is of critical importance for delay-sensitive applications; \textcolor{red}{And \SI{95}{\percent} bit rate reduction is reported when comparing the RAW image compression to the most popular JPEG coder at the same quality.} As such, the proposed $\rho$-Vision promises great potential for resource-efficient visual analytics. 
   %Executing tasks using RAW images is 
   %also attractive to applications having limited power consumption and stringent latency constraints because of the removal of redundant ISP. 
  % We will make our dataset and relevant materials publicly accessible later for reproducible research.% to encourage more interested parties to participate into this exciting exploration. 
   % \xzhang{What is the meaning of $\rho$ in $\rho$-Vision? -- $\rho$ is rho to mimic the pronunciation of RAW.}

\fi 



==> sections/comment/comment_compression.tex <==

\begin{comment}
\subsection{Near Lossless RIC}
Existing compression methods like LIC, are typically used VAE as their structure, where the entropy model corresponds to the prior on the latent representation. Since all transformations $E \left( \cdot \right)$ in the encoder are irreversible, it is difficult for the decoder to learn a perfect inverse transformation $D\left( \cdot \right)$ such that $\boldsymbol{x}\equiv D\left( E \left( \boldsymbol{x} \right) \right)$. As a result, they are unable to recover high quality images effectively which is important for RAW image compression that needs to be applied in film and video post-process. Besides, due to its irreversibility, the repeatedly compressed streams $b_i= \textrm{round} \left(E\left(D\left( \boldsymbol{b}_{i-1} \right)\right)\right)$ will not be the same as the initial one $\boldsymbol{b}_0= \textrm{round}\left(E\left(\boldsymbol{x}\right)\right)$, which means that the image $\boldsymbol{x}_i = D\left( \boldsymbol{b}_i \right)$ recovered by the $i^{th}$ compression at the same bit-rate is not the same as the image $\boldsymbol{x}_0 = D\left( \boldsymbol{b}_0 \right)$ recovered by the first compression. To solve this problem, we will introduce the invertible neural networks to replace the main encoder and main decoder in LIC. We have already introduced the invertible neural network in Sec.~\ref{sec:invISP}, and here we will elaborate the process in more detail. We assume that the invertible transformation $f$ consists of a series of invertible transformation functions $\left\{ f_0, f_1, \ldots, f_m\right\}$. Thus the encoding and decoding process could be written as:
\begin{align}
    \boldsymbol{b} &= f_m \circ \cdots  \circ f_1  \circ f_0 \circ \boldsymbol{x} \\
    \hat{\boldsymbol{b}} &= \textrm{round}(\boldsymbol{b}) \\
    \tilde{\boldsymbol{x}} &= f_0^{-1} \circ f_1^{-1} \circ \cdots \circ f_m^{-1} \circ \hat{\boldsymbol{b}}
\end{align}
The bijective function $f_i$ with input $\boldsymbol{m} \in \mathcal{R}^D$ and output $\boldsymbol{n} \in \mathcal{R}^D$ is implemented through affine
coupling layers, which formulated as:
\begin{align}
    \boldsymbol{n}_{1:d} &= \boldsymbol{m}_{1:d} \\
    \boldsymbol{n}_{d+1:D} &= \boldsymbol{m}_{d+1:D} \odot \exp{\left( s\left( \boldsymbol{n}_{1:d} \right)\right)} + t\left( \boldsymbol{n}_{1:d} \right),
\end{align}
where $s$ and $t$ represent scale and translation functions from $R^{d} \rightarrow R^{D-d}$, and $\odot$ is the Hadamard product.
For each $f_i$, the inverse process $f_i^{-1}$ can be written as:
\begin{align}
    \boldsymbol{m}_{1:d} &= \boldsymbol{n}_{1:d} \\
    \boldsymbol{m}_{d+1:D} &= \left( \boldsymbol{n}_{d+1:D} - t\left( \boldsymbol{m}_{1:d} \right) \right) \odot \exp{\left(-s\left( \boldsymbol{m}_{1:d} \right)\right)}
\end{align}
Also, the average pool is used as the down-sample method in the main encoder of rawLIC, which is irreversible. Instead, we use the rearrange operation and pixel-shuffle for down-sample and up-sample, respectively.
\end{comment}

\begin{comment}



let $\boldsymbol{Z}$

\begin{enumerate}
    \item First, we follow 
    
    prior $\boldsymbol{x}$ is derived by subtracting the original input  $\boldsymbol{x}_{file}$ from the  denormalizated reconstruction of lossy coded RAW image $\tilde{\boldsymbol{x}}_{file}$, e.g.,   $\boldsymbol{x}_{res} =  \tilde{\boldsymbol{x}}_{file}-\boldsymbol{x}_{file}$ having $\tilde{\boldsymbol{x}}_{file}$ generated by inverting \eqref{eq:linearization} and rounding.
    \item Then, a simple yet effective factorized entropy model $\textrm{Factor}\left( \theta \right)$~\cite{balle2018variational,minnen2018joint} is devised to compactly represent  $\boldsymbol{x}_{res}$. 
\end{enumerate}
%It is noticed that 
Note that rounding is not necessarily required for $\boldsymbol{x}_{res}$  since  $\boldsymbol{x}_{file}$ and $\tilde{\boldsymbol{x}}_{file}$ are both integers. 
Thus the $p\left(\boldsymbol{x}_{res} \right)$ could be calculated by $\textrm{Factor}\left(\boldsymbol{x}_{res}+0.5;~\theta\right)-\textrm{Factor}\left(\boldsymbol{x}_{res}-0.5;~\theta\right)$. 
Then we use AE to encode the residual into bitstream $\boldsymbol{b}_{res}= \textrm{AE}\left( \boldsymbol{x}_{res}, ~\textrm{Factor} \left( \theta \right) \right) $ while  for the decoding, $\boldsymbol{x}_{res}$ is decoded by $\textrm{AD}\left(\boldsymbol{b}_{res}, ~\textrm{Factor}\left( \theta \right) \right)$. As for training, we only need entropy loss $-log\left( p\left( \boldsymbol{x}_{res} \right)\right)$ since the compression is lossless on purpose.
%which make the decompressed $\hat{\boldsymbol{x}}_{file} \equiv \boldsymbol{x}_{file}$. Specifically, we first get the $\boldsymbol{x}$ from the normalized $\boldsymbol{x}_{file}$. And we take the pre-trained rawLIC to get the reconstructed image $\hat{\boldsymbol{x}}$ from $\boldsymbol{x}$. Then we get the rough $\tilde{\boldsymbol{x}}_{file}$ using de-normalization:
%\begin{align}
%&\tilde{\boldsymbol{x}}_{file} = \nonumber\\
%&\textrm{round}\left(  \left(\textrm{saturationLev}-\textrm{blackLev}\right) \hat{\boldsymbol{x}} + \textrm{blackLev}\right)
%\end{align}

%We use a factorized entropy model $\textrm{Factor}\left( \theta \right)$~\cite{balle2018variational,minnen2018joint} to represent the cumulative distribution function (CDF) of the residual $\boldsymbol{x}_{res} =  \tilde{\boldsymbol{x}}_{file}-\boldsymbol{x}_{file}$. It is noticed that $\boldsymbol{x}_{res}$ is not required to be rounded since $\tilde{\boldsymbol{x}}_{file}$ and $\boldsymbol{x}_{file}$ are both integers. Thus the $p\left(\boldsymbol{x}_{res} \right)$ could be calculated by $\textrm{Factor}\left(\boldsymbol{x}_{res}+0.5;~\theta\right)-\textrm{Factor}\left(\boldsymbol{x}_{res}-0.5;~\theta\right)$. Then we use arithmetic encoding $\textrm{AE}$ to encode the residual bit-stream $\boldsymbol{b}_{res}= \textrm{AE}\left( \boldsymbol{x}_{res}, ~\textrm{Factor} \left( \theta \right) \right) $. For the decoding side, the $\boldsymbol{x}_{res}$ is recovered by arithmetic decoding $\textrm{AD}\left(\boldsymbol{b}_{res}, ~\textrm{Factor}\left( \theta \right) \right)$. During training, we replace the recover loss in rawLIC to residual entropy loss $-log\left( p\left( \boldsymbol{x}_{res} \right)\right)$ since the recover process is lossless.

\end{comment}

==> sections/comment/comment_cycler2r.tex <==

% \Salnote{What do you want to say in this section/para, what is the topic sentence?} 
% Training supervised RAW-to-RGB  model via excessive RAW and RGB image pairs is straightforward~\cite{zamir2020cycleisp,abdelhamed2019noise,afifi2020cie} but impractical and cumbersome. 
% This is because the mapping between RAW and RGB images is not bijective due to the use of various camera sensors and diverse imaging settings (even for the same sensor).  The transformation from RGB images   $\mathcal{Y} = \{ \boldsymbol{y}_1,\boldsymbol{y}_2,\ldots, \boldsymbol{y}_i\}$ to the corresponding RAW images $\mathcal{X} = \{\boldsymbol{x}_{1}, \boldsymbol{x}_{2}, \ldots, \boldsymbol{x}_{i}\}$, commonly referred to as the inverse ISP (invISP), is an image-to-image translation problem. To avoid the desire of excessive paired RAW and RGB samples, and also to assure the model generalization across diverse camera sensors and imaging settings,  using unpaired data under an unsupervised training is greatly desired. \Salnote{We are repeating the message in the line above several times. We need to clearly describe it once and then talk about substantive contribution.}
% To tackle it, we propose to use the CycleGAN~\cite{zhu2017unpaired}  to guide the learning of respective mapping functions simultaneously, e.g., $g_{\rm invISP}$: RGB $\rightarrow$ RAW, and $f_{\rm ISP}$: RAW to $\rightarrow$ RGB. We call it Unpaired CycleR2R for short.
% Note that the CycleGAN has been already used for tasks like style transfer and object transfiguration with remarkable performance~\cite{zhu2017unpaired}. 
%More details can be found  at \url{https://junyanz.github.io/CycleGAN/}. 

%We therefore forumate the mapping from 
%difference
%because: 1) excessive amount of image pairs are required for various camera sensors; 2) even for the same senor, acquired RAWs can be different for the same scene due to the diverse imaging settings like color temperature, exposure, color correction, etc. 

%We basically want to convert RGB images  $\mathcal{Y} = \left\{ \boldsymbol{y}_1, ~\boldsymbol{y}_2,~ \ldots, ~\boldsymbol{y}_i, ~\ldots \right\} $ to corresponding RAW representations  $\mathcal{X}_t = \left\{\boldsymbol{x}_{t_1}, ~\boldsymbol{x}_{t_2}, ~\ldots, ~\boldsymbol{x}_{t_i}, ~\ldots \right\}$

%The RGB-to-RAW mapping, which is also referred to as the inverse ISP (invISP), is to generate the linear RAW images $\mathcal{X}^t = \left\{\boldsymbol{x}^t_{1}, \boldsymbol{x}^t_{2}, \ldots, \boldsymbol{x}^t_{i}, \ldots \right\}$  \xzhang{for a target camera Cam$^t$} from a serial RGB images  $\mathcal{Y} = \left\{ \boldsymbol{y}_1,\boldsymbol{y}_2,\ldots, \boldsymbol{y}_i,\ldots \right\}$. \maz{Note that \xzhang{the} imaging setting, \eg, acquisition device, exposure, etc, may not be available along with the existing RGB datasets. Thus, we usually define \xzhang{the target} camera Cam$^t$ to have simulated RAW samples best imitating its characteristics learned from native RAWs acquired in practice. All native RAWs captured by real-life cameras in this paper are normalized using black level blackLev and saturation level saturationLev from the EXIF data for the sake of simplicity. Later, we also offer the RAW-to-RAW transfer to ensure the generalization for various camera sensors.}

%The purpose our inverse ISP is to convert a serious of images $\mathcal{Y} = \left\{ \boldsymbol{y}_1, ~\boldsymbol{y}_2,~ \ldots, ~\boldsymbol{y}_i, ~\ldots \right\} $ from the RGB dataset into the linear RAW images $\mathcal{X}^t = \left\{\boldsymbol{x}^t_{1}, ~\boldsymbol{x}^t_{2}, ~\ldots, ~\boldsymbol{x}^t_{i}, ~\ldots \right\}$ captured by target camera $\textrm{Cam}^t$. It is noted that all RAW images in this paper have been normalized using black level and saturation from the EXIF data for the sake of simplicity.

%Assume that $\boldsymbol{y}_i$ is rendered from $\boldsymbol{x}^s_{i}$ through $\textrm{ISP}^{s}$, which is designed by the manufacture of camera $\textrm{Cam}^s$. The conversion between the RAW images captured by $\boldsymbol{x}^s_{i}$ and $\boldsymbol{x}^t_{i}$ could be modeled by a linear conversion which is the first step of ISP. Therefore, we assume that there exists an  $\textrm{ISP}^{t}$ that can convert $\boldsymbol{x}^t_{i}$ to $\boldsymbol{y}_i$ which means we could get $\boldsymbol{x}^t_{i}$ through inverse ISP $\textrm{invISP}^{t}\left( \boldsymbol{y}_i \right)$. 


%Although current invISPs based on neural networks have achieved satisfactory results on tasks such as denoising~\cite{zamir2020cycleisp, abdelhamed2019noise} and HDR recovery~\cite{xing2021invertible}, all of them rely on a large number of paired RAW-RGB images which are not accessible in most of published RGB datasets. But we can capture 
% \xzhang{capture??} 
%lots of $\widetilde{\mathcal{X}}^t = \left\{ \tilde{\boldsymbol{x}}^t_{1}, \tilde{\boldsymbol{x}}^t_{2},\ldots,\tilde{\boldsymbol{x}}^t_{j},\ldots\right\} $ with the $\textrm{Cam}^{t}$. So we want to model the $\textrm{invISP}^{t}$ within unpaired RAW and RGB, \ie, $\left \{ \widetilde{\mathcal{X}}^t, ~\mathcal{Y} \right \}$. It is worth noting that $\textrm{ISP}^{t}$ is not an bijective function, \eg the various of RAW images captured in the same scene at different color temperatures will have the same RGB image because of the auto white balance. In other words, for $\textrm{invISP}^{t}$, the same input should have several outputs.



%\maz{To this aim, this work devises stacked five convolutional layers to form   $E_{wb}\left( \cdot \right)$ model for fulfill the $f_{wb}$. the derivation of $\omega_i$, $r_i$ and $b_i$.}


%\maz{}.

%\maz{The proposed $E_{wb}\left( \cdot \right)$ accepts paired inputs as aforementioned to derive the weight, \eg,
%\begin{align}\label{eq:w_i}
%    w_i &=  E_{wb} \left( \left\{\hat{\boldsymbol{x}}_{wb_i}, ~\hat{\boldsymbol{x}}^2_{wb_i}  \right\} \right),
%\end{align} and  produce the final gain for AWB as defined in \eqref{eq:white_balancing}.
%}

\begin{comment}
We will simulate this process with a basic encoder $E_{wb}$. And since we do not have access to the parameters of $\textrm{Cam}^t$, we set the $\left\{R_{gain}, ~B_{gain} \right\}$ as the learnable parameters shared by $\textrm{ISP}^t$ and $\textrm{invISP}^{t}$ following ~\cite{conde2022model}.

The basic encoder $E_{wb}\left( \cdot \right)$ consists of several layers. The first layers designed as a 5$\times$5 convolution to expand the perceptual field to obtain global information. The subsequent two layers use the combination of 3$\times$3 convolution and leaky ReLU to reduce the computational workloads. The final two layers are linear layers used to regress the coefficients $w_{i} \in W$. Since the color temperature estimation does not require detailed information, and to reduce the computational effort, we first downsample the input $\boldsymbol{x}_{demo}$ to 128$\times$128 noted as $\boldsymbol{x}^{\downarrow}_{demo}$. 
% Afterwards, considering that $\left\langle r_{gain_i}, ~b_{gain_i} \right\rangle$ are constantly updated during the training process, the network does not know what $\left\langle r_{gain_i}, ~b_{gain_i} \right\rangle$ is at this moment if the images are input directly. Therefore, instead of putting image directly, 
Then we use the pre-white balanced image $ \hat{\boldsymbol{x}}_{wb_i} = \left( r_{i}, ~1, ~b_{i} \right) \cdot \boldsymbol{x}^{\downarrow}_{demo}$ and its extracted feature $\hat{\boldsymbol{x}}_{wb_i}^2$ as the input of $E_{wb}\left( \cdot \right)$ to obtain the corresponding coefficients $w_i$. And the final gain $\left(r_{gain}, ~b_{gain}\right)$ is obtained by $\sum_{i} w_{i}\cdot\left( r_{i}, ~b_{i} \right)$ as same as the camera inner ISP. And the final gain $\left(r_{gain}, ~b_{gain}\right)$ is obtained by $\sum_{i} w_{i}\cdot\left( r_{i}, ~b_{i} \right)$ as same as the camera inner ISP.

If multiplying $\left( r_{gain_i}, ~1, ~g_{gain_i} \right) $ directly to $\boldsymbol{x}_{demo}$ would led to highlight overflow, we 
used the safty gain function $S\left( \boldsymbol{x}, ~gain\right)$ in UPI~\cite{brooks2019unprocessing} to retaining highlights.

%we augment the $\left( r_{gain_i}, ~1, ~g_{gain_i} \right)$ to 


% ,
% which could be written as:
% \begin{align}
%     \boldsymbol{\alpha} &= \max \left( \frac{\boldsymbol{x}-\eta}{1-\eta} , ~0\right) \\
%     S\left(\boldsymbol{x}, ~gain\right) &= \max \left( gain \cdot (1-\boldsymbol{\alpha}^2) \odot \boldsymbol{x}, ~\boldsymbol{x} \right)
% \end{align}
% , where $\odot$ is the Hadamard product and $\eta$ is the hyper-parameter using to deteminate the highlight part which we set to $0.9$.
The whole process of our AWB model could be formulated as:
\begin{align}
    \hat{\boldsymbol{x}}_{wb_i} & =  ~\left( r_{i}, ~1, ~b_{i} \right) \cdot \boldsymbol{x}_{demo}^{\downarrow} \\
    w_i &=  E_{wb} \left( \left\{\hat{\boldsymbol{x}}_{wb_i}, ~\hat{\boldsymbol{x}}^2_{wb_i}  \right\} \right) \\
    \left( r_{gain}, ~b_{gain}\right) &= \sum_i w_i \cdot \left( r_{i}, ~b_{i} \right) \\
    % \boldsymbol{x}_{wb}&=
    f_{wb} \left( \boldsymbol{x}_{demo} \right) &= S\left(\boldsymbol{x}_{demo}, ~\left( r_{gain}, ~1, ~b_{gain}\right)  \right)
\end{align}
\end{comment}
% More over, for better extraction of color features, we manually designed pre-extracted features $ \hat{\boldsymbol{x}}^2_{wb_i}$ and concatenate it with the $\hat{\boldsymbol{x}}_{wb_i}$ into the network.





% wide range 


% same scene captured within a wide range of exposure level will get the similar image after the brightness adjustment, 
% plotz2017benchmarking

% To avoid the output $b$ of the $E_{b}\left( \cdot \right)$ being too large and affecting the training stability, we manually scaled the value to


\begin{comment}
Specifically, the entire process to adjust brightness of a white-balanced image $x_{wb}$, could be formulated as:

\begin{align}
     b &= E_{b}\left( G \left( \boldsymbol{x}_{wb}^{\downarrow} \right) \right) \\
    %  \boldsymbol{x}_b &= 
     f_{b}\left( \boldsymbol{x}_{wb} \right) &= S\left( \boldsymbol{x}_{wb}, ~gain \right)
\end{align}
, where $\alpha$ and $\beta$ are used to limit the range of brightness adjustment which we set as 0.2 and 0.8.
At the same time, $f_{b}$ is also a non-injective function, in other words, the same scene captured within a wide exposure range will get the similar image after the brightness adjustment. Therefore, We use the Gaussian distribution $\mathcal{N} \left( \mu_b, ~\sigma^2_b \right)$ to measure this range. For a image $x_b$ with adjusted brightness, we use $E^{-1}_{b}\left( \cdot \right)$ to estimate the mean and variance of its original exposure level. So the whole $g_{b}$ can be written as:
\begin{align}
    \mu_b, ~\sigma_b &= E^{-1}_{b} \left( G\left(  \boldsymbol{x}_b^{\downarrow} \right) \right) \\
    g_{b}\left( \boldsymbol{x}_b \right) &= \boldsymbol{x}_b \cdot gain, ~gain\sim{\mathcal{N}\left( \beta+\mu_b, ~\sigma^2_b \right)}
\end{align}
\end{comment}

%Since the response of the camera to different spectral is different from the human eye, cameras will apply a $3\times3$ color correction matrix (CCM) in order to convert its own color space to the human's, \eg sRGB~\cite{afifi2020cie}.
% ISP need the color correction to convert the an image $x_b$ that matches the response curve of the human eye. Because the spectral space is a linear space, the color correction can be represented by a $3\times3$ matrix, noted as color correction matrix (CCM). 

%generate  $\mu_d/\mu_n$ a

%that $\omega_d^{-1}/\omega_n^{-1}$ follows a Gaussian distribution $\mathcal{N}\left( \mu_d/\mu_n, ~\sigma_d^2/\sigma_n^2 \right)$ where mean $\mu_d/\mu_n$ and variance $\sigma_d^2/\sigma_n^2$ are generated by $E_{cc}^{-1}\left(\cdot\right)$ shared the same architecture of $E^{-1}_{wb}\left(\cdot\right)$. 


%Inverting$w_$ this process from $\boldsymbol{x}_{cc}$ is also challenging because, the same color corrected image may derive from a variety of mixed illumination and therefore the $\omega_d^{-1}/\omega_n^{-1}$ is uncertain. However, similar to $g_{wb}$, we can assume that $\omega_d^{-1}/\omega_n^{-1}$ follows a Gaussian distribution $\mathcal{N}\left( \mu_d/\mu_n, ~\sigma_d^2/\sigma_n^2 \right)$ where mean $\mu_d/\mu_n$ and variance $\sigma_d^2/\sigma_n^2$ are generated by $E_{cc}^{-1}\left(\cdot\right)$ shared the same architecture of $E^{-1}_{wb}\left(\cdot\right)$. Thus, the generation of $\omega_d^{-1}/\omega_n^{-1}$ can be expressed as followed:
%\begin{align} 
%    \left\{\mu_d/\mu_n, ~\sigma_d/\sigma_n\right\} &= E^{-1}_{cc} \left( \left\{ \hat{\boldsymbol{x}}_{d}/\hat{\boldsymbol{x}}_{n}, ~\hat{\boldsymbol{x}}_{d}^2/\hat{\boldsymbol{x}}_{n}^2 \right\}\right), \\
%    \omega_d^{-1}/\omega_n^{-1}&\sim{\mathcal{N}\left( \mu_d/\mu_n, ~\sigma_d^2/\sigma_n^2 \right),}
%\end{align}
%where $\hat{\boldsymbol{x}}_{d}/\hat{\boldsymbol{x}}_{n}$ is augmented input derived by multiplying $\textrm{CCM}_d^{-1}/\textrm{CCM}_n^{-1}$ to $\boldsymbol{x}^{\downarrow}_{cc}$. Then given pseudo-inverse matrix, \eg, 
%\begin{align}
%\textrm{CCM}_{mix}^{-1}=\left( \omega_d^{-1} \textrm{CCM}_d + \omega_n^{-1} \textrm{CCM}_n \right)^{-1},
%\end{align}
%the inverse color correction could be written as:


\begin{comment}

Considering that images taken in both daylight and nighttime are converted to the same color space after $f_{cc}$, the inverse process $g_{cc}$ should also be a one-to-many function. We assume the combination coefficient $k_{d}$ and $k_{n}$ are following the Gaussian distribution modeled by $E_{cc}^{-1} \left( \cdot \right)$, then
% Then the inverse CCM can also be written as $\textrm{CCM}_{comb}^{-1}=k_{d}\cdot \textrm{CCM}^{-1}_{d}+k_{n}\cdot \textrm{CCM}^{-1}_{n}$, where $k_{d}\sim{\mathcal{N}\left( \mu_{d}, ~\sigma^2_{d} \right)}, ~k_{n}\sim{\mathcal{N}\left( \mu_{n}, ~\sigma^2_{n} \right)}$, and the $\mu_d, ~\sigma_d, ~\mu_n, ~\sigma_n$ are generated by a neural network $E^{-1}_{cc} \left( \cdot \right)$.
% To summarize, 
% its inverse process the 
$g_{cc}$ to convert color corrected image $\boldsymbol{x}_{cc}$ can be expressed as:
\begin{align}
    \left\{ \hat{\boldsymbol{x}}_{d}, ~\hat{\boldsymbol{x}}_{n} \right\}& = \left\{ \textrm{CCM}_d^{-1}, ~\textrm{CCM}_n^{-1} \right\} \cdot \boldsymbol{x}_{cc}^{\downarrow} \\
    % x_d &= x_{cc} \cdot CCM_d^{-1} \\
    % x_n &= x_{cc} \cdot CCM_n^{-1} \\
\begin{split}  
    \mu_d, ~\sigma_d &= E^{-1}_{cc} \left( \left\{ \hat{\boldsymbol{x}}_{d}, ~\hat{\boldsymbol{x}}_{d}^2 \right\} \right) \\
    \mu_n, ~\sigma_n &= E^{-1}_{cc} \left( \left\{ \hat{\boldsymbol{x}}_{n}, ~\hat{\boldsymbol{x}}_{n}^2 \right\} \right) 
\end{split}
\\
    \begin{split}
        \textrm{CCM}_{comb}^{-1} &= k_d \cdot \textrm{CCM}_d^{-1} + k_n \cdot \textrm{CCM}_n^{-1}, \\
        &\quad~ k_{d}\sim{\mathcal{N}\left( \mu_{d}, ~\sigma^2_{d} \right)}, ~k_{n}\sim{\mathcal{N}\left( \mu_{n}, ~\sigma^2_{n} \right)}
    \end{split}\\
    g_{cc}\left( \boldsymbol{x}_{cc} \right) &= \textrm{CCM}_{comb}^{-1} \cdot \boldsymbol{x}_{cc}
\end{align}
\end{comment}


\begin{comment}

to implement this process, so the transformation $f_{gamma}$ and inversion $g_{gamma}$ can be represented as:
\begin{align}
\begin{split}
    \f_{gamma}\left( \boldsymbol{x}_{cc} \right) &=\left\{
        \begin{aligned}
            &12.92\cdot \boldsymbol{x}_{cc}, &\boldsymbol{x}_{cc} \leq 0.00304\\
            &1.055\cdot \boldsymbol{x}_{cc}^{1/2.4}-0.055, &\boldsymbol{x}_{cc}>0.00304
        \end{aligned}
    \right.
\end{split}
\\
\begin{split}
    g_{gamma} \left(\boldsymbol{x}_{g} \right) &=\left\{
        \begin{aligned}
            &\frac{\boldsymbol{x}_{g}}{12.92}, &\boldsymbol{x}_{g} \leq 0.04045\\
            &\left(\frac{\boldsymbol{x}_{g}+0.055}{1.055}\right)^{2.4}, &\boldsymbol{x}_{g} > 0.04045
        \end{aligned}
    \right.
\end{split}
\end{align}
\end{comment}

\begin{comment}
\subsubsection{Local Transforms}
% \begin{figure}
%      \centering
%      \includegraphics[width=0.7\linewidth]{Figs/invertible_transformation.pdf} 
%      \caption{{\bf Local Transform.} Our local transform is implemented using the invertible transformation where $E_c$\zhihao{amend this figure $E_l\rightarrow E_c$}, $E_s$ and $E_t$ are Residual Block~\cite{he2016deep}.}
%      \label{fig:local_transform}
% \end{figure}


Most ISPs enhance image details with a serial local transformations like tone mapping, sharpening, contrast adjustment, etc. To simulate these complex transformations,  e.g., $f_{local}$ in ISP and $g_{local}$ in invISP, one approach is to train two separate CNN models respectively~\cite{zamir2020cycleisp, afifi2020cie}, which, however, often leads to $\hat{\boldsymbol{x}}_{g} \neq g_{local} \circ f_{local} \circ \boldsymbol{x}_{g}$ due to the nonlinear computations involved in CNNs. {Though nonlinear computations are also used in AWB, brightness adjustment, color correction, they are global operations which do not directly incur the loss of local details. Furthermore, %as revealed subsequently, 
our CycleGAN-based framework iterates the source-target translation in training which would greatly accumulate the loss of details and severely deteriorate the training stability.}

To tackle it, we propose to use generative flow based invertible neural network (INN)~\cite{kingma2018glow} to assure $\boldsymbol{x}_{g} \equiv  g_{local} \circ f_{local} \circ \boldsymbol{x}_{g}$.
Specifically,  we first split $\boldsymbol{x}_{g}$ into respective Red, Green, Blue channels $\left\{\boldsymbol{r}, ~\boldsymbol{g}, ~\boldsymbol{b}\right\} \in \mathbb{R}^{h \times w \times 1}$ with $h$ and $w$ as the height and width of $\boldsymbol{x}_{g}$. Next  local transformed $\hat{\boldsymbol{g}}$ is derived by
\begin{align}\label{local_g}
    \hat{\boldsymbol{g}} = \boldsymbol{g} + E_c\left( \left\{ \boldsymbol{r}, ~\boldsymbol{b} \right\} \right), 
\end{align} with channel merging function $E_{c}\left( \cdot \right): \mathbb{R}^{h\times w \times 2} \rightarrow \mathbb{R}^{h \times w \times 1}$ used to combine $\bf r$ and $\bf b$.
Then $\hat{\boldsymbol{r}}, ~\hat{\boldsymbol{b}}$ are respectively computed using a scaling function $E_s\left( \cdot \right)$ and a  channel expansion $E_t\left( \cdot \right): \mathbb{R}^{h\times w \times 1} \rightarrow \mathbb{R}^{h \times w \times 2}$, i.e.,
\begin{align}\label{local_rb}
    \left\{ \hat{\boldsymbol{r}}, ~\hat{\boldsymbol{b}} \right\} &= \left\{ \boldsymbol{r}, ~\boldsymbol{b} \right\} \odot
        \exp{ \left( E_{s} \left( \hat{\boldsymbol{g}} \right) \right)} +
        E_{t} \left( \hat{\boldsymbol{g}} \right),
    % \boldsymbol{y} &= f_{local} \circ \boldsymbol{x}_g  = \left\{\hat{\boldsymbol{r}}, ~\hat{\boldsymbol{g}}, ~\hat{\boldsymbol{b}}\right\},
\end{align}
where $\odot$ is the Hadamard product, %\zhihao{according to \href{https://stats.stackexchange.com/questions/533577/what-is-the-difference-between-the-dot-product-and-the-element-by-element-multip}{stack overflow} and \href{https://en.wikipedia.org/wiki/Hadamard_product_(matrices)}{wiki},} 
 Finally, $\boldsymbol{y}$ is generated accordingly:
\begin{align}
    \boldsymbol{y} = f_{local} \circ \boldsymbol{x}_{g} = \left\{ \hat{\boldsymbol{r}},~\hat{\boldsymbol{g}},~\hat{\boldsymbol{b}}  \right\}. \label{local_y}
\end{align}

Reversely, given the $\left\{ \hat{\boldsymbol{r}},~\hat{\boldsymbol{g}},~\hat{\boldsymbol{b}} \right\}$ of $\boldsymbol{y}$, $ g_{local}$   inverts the process of (\ref{local_g})-(\ref{local_y}) of $f_{local}$ to derive the $\boldsymbol{x}_g$, e.g.,
\begin{align}
    \left\{ \boldsymbol{r}, ~\boldsymbol{b} \right\} &= \left( \left\{ \hat{\boldsymbol{r}}, ~\hat{\boldsymbol{b}} \right\} - E_t \left( \hat{\boldsymbol{g}} \right) \right)
        \odot 
        \exp{ \left( -E_s\left( \hat{\boldsymbol{g}} \right) \right)}, \\
    \boldsymbol{g} &= \hat{\boldsymbol{g}} - E_c\left( \left\{ \boldsymbol{r}, ~\boldsymbol{b} \right\} \right),\\
    \boldsymbol{x}_{g} &= g_{local} \circ \boldsymbol{y} = \left\{\boldsymbol{r}, ~\boldsymbol{g}, ~\boldsymbol{b} \right\}.
\end{align}

Both $ g_{local}$ and $ f_{local}$  are illustrated in the supplemental material. Other solutions for INN can be also applied as well. Here we just give an example using the generative flow~\cite{kingma2018glow}. 
\end{comment}


\begin{comment}
\subsection{RAW-to-RAW Mapping for Model Generalization}
\label{sec:raw_data_aug}
%\maz{revisit!!}
Having the proposed Unpaired CycleR2R, we can easily convert any RGB images $\mathcal{Y}$ to the corresponding RAW samples $\mathcal{X}^{t}$ by learning the characterization from limited RAW snapshots of a specific target camera $\text{Cam}^{t}$. In cameras, various types of sensors can be used; while even for the same sensor, diverse imaging settings may be applied. A naive way is to collect a new set of RAW images to properly retrain the Unpaired CycleR2R. As revealed by our simulations, it takes about several hours to execute such task by enforcing 20,000 training iterations~\cite{zhu2017unpaired}.

%\maz{How many RAW images are required? Fewer RAWs leads to faster re-traning? What about the size of RGB dataset? If we are using ImageNet1K, will it be longer than CityScapes?}

%\zhihao{We always train 20,000 iterations, independent of the RGB/RAW dataset size.}

%, leading to sensor-specific RAW representations. Of course, we can refine the Unpaired CycleR2R specifically for different scenarios, which however, is cumbersome and impractical for model deployment. 

Alternatively, we offer a lightweight solution for the same purpose. The problem of model generalization is mainly due to the reason that RAW images are sensor-specific~\cite{afifi2020cie}.
Recently, a seminal work by Afifi \etal.~\cite{afifi2020cie} showed that any sensor-specific RAWs  could be linearly transformed to sensor-independent CIE XYZ images. It then motivates us to use CIE XYZ space as the common intermediate format for transformation:
\begin{enumerate}
    \item  We first convert RAWs  $\mathcal{X}^{t}$ corresponding to the $\text{Cam}^{t}$ to XYZ images $\mathcal{Z}$, for which it sequentially invovles the bilinear demosaicing defined in \eqref{eq:demosaic}, AWB in~\eqref{equation:wb} through the use of gains suggested by~\cite{van2007edge}, brightness adjustment as in~\eqref{equation:brightness} with $b_{gain}$ randomly-sampled from $\mathcal{N}\left( 0.8, ~0.3\right)$ following~\cite{brooks2019unprocessing}, and color correction as in \eqref{equation:ccm} by  linearly weighting the CCM presets;
    \item To convert $\mathcal{Z}$ to  $\mathcal{X}^{n}$ characterized by the $\text{Cam}^{n}$,  we reverse the color correction, brightness adjustment, AWB and demosaic steps. 
Specifically, we first invert the color correction of $\mathcal{Z}$ using \eqref{equation:inv_ccm} with random CCM presets from $\text{Cam}^{n}$, and then follow \eqref{equation:inv_brightness} to do brightness adjustment with $b_{gain}$ randomly sampled from $\mathcal{N}\left( 0.8, ~0.3\right)$ which is same as the forward processing.  Final $\mathcal{X}^{n}$ is produced by mosaicing the output of \eqref{equation:inv_wb}, where AWB gain is derived by randomly-sampled $\text{Cam}^{n}$ presets. 
\end{enumerate}

As seen, we do not require any retraining for RAW to RAW mapping across different cameras; and having the  CIE XYZ space as the intermediate state for transformation can greatly speed up the process.

\end{comment}

%$D_{local}$ processes the images 

%First, we set the RGB images $\mathcal{Y}$ as the source domain and RAW images $\widetilde{\mathcal{X}}^t$ as the target. 
% Then we use the $\textrm{invISP}^t$ and $\textrm{ISP}^t$ as the the source-to-target and target-to-source generator, respectively. 
%Then we use the $\textrm{invISP}^t$ to convert a RGB image $\boldsymbol{y} \in \mathcal{Y}$ to its RAW format $\hat{\boldsymbol{x}}^t$ and the $\textrm{ISP}^t$ to render a RAW image $\tilde{\boldsymbol{x}}^t \in \widetilde{\mathcal{X}}^t$ to its RGB representation $\hat{\boldsymbol{y}}$. 
%Finally, 
%for the purpose of distinguishing the real RGB/RAW $\boldsymbol{y}/\tilde{\boldsymbol{x}}^t$ and generated $\hat{\boldsymbol{y}}/\hat{\boldsymbol{x}}^t$, 
%we propose a discriminator $D_{rgb}/D_{raw}$ to distinguish the real RGB/RAW $\boldsymbol{y}/\tilde{\boldsymbol{x}}^t$ and the generated $\hat{\boldsymbol{y}}/\hat{\boldsymbol{x}}^t$.
%we propose one discriminator $D_{rgb}$ to distinguish the real RGB $\boldsymbol{y}$ and the generated $\hat{\boldsymbol{y}}$, and another discriminator $D_{raw}$ to distinguish the real 
%RAW $\tilde{\boldsymbol{x}}^t$ and the generated $\hat{\boldsymbol{x}}^t$.



%Both the $D_{raw}$ and $D_{rgb}$ consist of three parts: $D_{local}$, $D_{color}$ and $D_{bright}$. Similar to the most image translation works~\cite{zhu2017unpaired, creswell2018generative, brock2018large, mao2017least}, $D_{local}$ is introduced to make sure that each pixel can be supervised to ensure the quality of generated image. Notably, even though the $D_{local}$ could supervise $f_{local}$ and $g_{local}$ well, it fails in perceiving the color and brightness of the whole image which is indispensable for $f_{wb},~f_{cc}, ~f_{b}, ~g_{wb}, ~g_{cc}$ and $g_{b}$ because of its perceptual field restriction. Inspired by FFCC~\cite{barron2017fast}, we propose the $D_{color}$ taking the log-chroma transformed image as input to discriminate the color distribution between the real image and generated. In order to tell apart the difference of global brightness, we feed the histogram of image into a brightness discriminator $D_{bright}$. The architecture of $D_{local}$ and $D_{color}$ consists of five convolution layers with Leaky ReLU~\cite{xu2015empirical} activation function. Since the input of $D_{bright}$ is an one-dimensional histogram, the convolution layers is replaced by linear layers. Hence their outputs are added directly to derive the final output of the discriminators $D_{rgb}$ and $D_{raw}$.

%\subsubsection{Loss Function}
%Typically, after the procession of an image transforming from RGB to RAW and then rendering it back, we should obtain the same one since ISP is a surjection function.

%if we transform a RGB image to its RAW counterpart and then leverage ISP to process the RAW image, we can get back the original RGB image, and vice versa.
% Under the CycleGAN framework, we attempt to simultaneously optimize the quality of both generated RAW image and generated RGB image. 
%To this end, we %incentivize this behavior with  define the cycle consistency loss $\mathcal{L}_{cycle}$ with the aim of  reserving high fidelity of details during the generation. Specifically, we expect the re-generated RGB image $\overline{\boldsymbol{y}} = \textrm{ISP}^t \left( \hat{\boldsymbol{x}}^t \right)$ to be consistent with the real $\boldsymbol{y}$.  Meanwhile, due to the invariant characteristic of image content, the re-generated RAW image $\overline{\boldsymbol{x}}^t = \textrm{invISP}^t \left( \hat{\boldsymbol{y}} \right)$ and $\tilde{\boldsymbol{x}}^t$ should be as close as possible to each other. Consequently, we follow the CycleGAN~\cite{zhu2017unpaired} using $\mathcal{L}_1$-norm to reduce these gap:
%\begin{equation}
%    \mathcal{L}_{cycle} = \Vert \overline{\boldsymbol{y}} - \boldsymbol{y} \Vert_{1} 
%    + \lambda_{raw} \cdot \Vert \overline{\boldsymbol{x}}^t  - \tilde{\boldsymbol{x}}^t \Vert_{1} .
%\end{equation}
%Considering that the $\textrm{invISP}^t$ is a one-to-many function making color and brighntess differences between $\overline{\boldsymbol{x}}_t$ and $\tilde{\boldsymbol{x}}^t$, we set the $\lambda_{raw}$ to a small value, \ie, 0.1.

\begin{comment}

We convert U, V

Adversarial loss $\mathcal{L}_{adv}$~\cite{mao2017least}, \ie,
\begin{align}
\mathcal{L}&_{adv} =  \nonumber\\
&\Vert 1 - D_{raw}( g_{\rm invISP}({\boldsymbol{y}}) )  \Vert_2
        + \left \Vert 1 - D_{rgb}\left( f_{\rm ISP}({\boldsymbol{x}}) \right) \right \Vert_2,
\end{align} is also augmented to have the final loss in generator as:
\begin{equation}
    \mathcal{L}_{G} = \mathcal{L}_{cycle} + \lambda_{adv} \cdot \mathcal{L}_{\text{adv}},
\end{equation}
where $\lambda_{adv}$ = 0.1 following the suggestion in~\cite{zhu2017unpaired}.

Similarly, loss function in discriminator is formulated as
%, since $D_{raw}$ and $D_{rgb}$ are designed for distinguishing between real image $\boldsymbol{y}/\tilde{\boldsymbol{x}}^t$ and generated $\hat{\boldsymbol{y}}/\hat{\boldsymbol{x}}^t$, we apply discriminator loss:
\begin{align}
\begin{split}
    \mathcal{L}_{D} &=  \left \Vert 1 - D_{raw}\left( {\boldsymbol{x}}  \right) \right \Vert_2
            + \Vert D_{raw} ( g_{\rm invISP}({\boldsymbol{y}})  ) \Vert_2 \\
        &+  \left \Vert 1 - D_{rgb}\left( \boldsymbol{y}  \right) \right \Vert_2
            +  \left \Vert D_{rgb}\left( f_{\rm ISP}({\boldsymbol{x}}) \right) \right \Vert_2.
\end{split}
\end{align}


Details regarding the setup of CycleGAN is given in~\cite{zhu2017unpaired}.

\end{comment}

==> sections/figures/r_classification_zero_shot_visual.tex <==
% \newcolumntype{M}[1]{>{\centering\arraybackslash}p{#1}}


\newcommand{\AddClsImg}[2]{\includegraphics[width=#1\textwidth]{#2}}
% 
\newcommand{\AddClsImgs}[4]{
\multirow{-3}{*}{\rotatebox[origin=c]{90}{\textbf{#4}}} \quad&
\AddClsImg{0.145}{Figs/classification_zero_shot_visual/#1/#2_w_label.png} &
\AddClsImg{0.145}{Figs/classification_zero_shot_visual/#1_clean_input/#2_w_label.png} &
\AddClsImg{0.145}{Figs/classification_zero_shot_visual/#1/#2_Conv2d_0_channel_#3.png} &
\AddClsImg{0.145}{Figs/classification_zero_shot_visual/#1_clean_input/#2_Conv2d_0_channel_#3.png} &
\AddClsImg{0.145}{Figs/classification_zero_shot_visual/#1/#2_gradcam.png} &
\AddClsImg{0.145}{Figs/classification_zero_shot_visual/#1_clean_input/#2_gradcam.png}
}

\newcommand{\AddDirtypix}[1]{
\AddClsImgs{joint_real_2to200lux}{#1}{22}{RGB}
}

\newcommand{\AddinvISP}[1]{
\AddClsImgs{invISP_2to200lux}{#1}{29}{RAW}
}


\begin{figure*}
\begin{center}
% \begin{tabular}{p{0.145\textwidth}@{ } p{0.145\textwidth}@{ } p{0.145\textwidth}@{ } p{0.145\textwidth}@{ } p{0.145\textwidth}@{ } p{0.145\textwidth}@{ }}
\begin{tabular}{c@{} c@{ } c@{ } c@{ } c@{ } c@{ } c@{ }}
&
\multicolumn{2}{c}{\textbf{Input Image}}
& 
    \multicolumn{2}{c}{\textbf{Noise Channel}}

& 
    \multicolumn{2}{c}{\textbf{Grad-CAM}}
\\
& Noise
& Clean
& 
    w/ Noise Input
& 
    w/ Clean Input
&
    w/ Noise Input
& 
    w/ Clean Input
\\

\AddDirtypix{IMG_20180314_190359}
\\
\AddinvISP{IMG_20180314_190359}
\\ 
\midrule
\AddDirtypix{IMG_20180314_200348}
\\
\AddinvISP{IMG_20180314_200348}
\\ 

% \AddDirtypix{IMG_20180314_200620}
% \\
% \AddinvISP{IMG_20180314_200620}
% \\ 

% \makecell{noise input} & \makecell{clean input} & \makecell{noise channel \\ (w/ noise input)} & \makecell{noise channel \\ (w/ clean input)} & \makecell{grad-cam \\ (w/ noise input)} & \makecell{grad-cam \\ (w/ clean input)} \\


\end{tabular}
\end{center}
\caption{\textbf{Visualization of classifier response to noisy and clean inputs using Anscombe ISP~\cite{diamond2021dirty} and direct RAW input.} Odd columns depict RGB inputs processed through Anscombe ISP and the resulting classifications by an RGB-domain classifier. Even columns show the corresponding classifications by a RAW-domain classifier using direct RAW inputs. The ``Noise Channel" represents the feature channel with the maximum difference between the noise input and clean input at the shallow layer ``Conv2d\_0" of the network. The Grad-CAM~\cite{selvaraju2017grad} visualizations are based on the last convolutional layer ``Conv2d\_13\_pointwise". A comparison between the ``Noise Channel" under different inputs reveals that the RAW-domain classifier is adept at extracting noise patterns, effectively separating noise from the signal, which results in Grad-CAM visualizations that more closely resemble the clean input. In contrast, the RGB-domain classifier struggles to disentangle noise from the signal due to the complex non-linear processing by the Anscombe ISP, leading to significant deviations in Grad-CAM under noisy conditions and consequently to misclassification.}
\label{figure:r_classification_zero_shot_visual}
\end{figure*}

\renewcommand{\arraystretch}{1} % 调整这个值

==> sections/figures/r_detection_compare_visual.tex <==
% \newcolumntype{M}[1]{>{\centering\arraybackslash}p{#1}}


\newcommand{\AddDetImg}[2]{\includegraphics[width=#1\textwidth]{#2}}
% 
\newcommand{\AddDetImgs}[2]{
\AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/ldr_raw.png} &
\AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/hdr_raw.png} &
\AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/rgb.png}
}



\begin{figure*}
\begin{center}
% \begin{tabular}{p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ }}
\begin{tabular}{c@{ } c@{ } c@{ }}
\multicolumn{3}{c}{Facing the Sun} \\
\AddDetImgs{face_sun}{2021-09-11-0800_0-CapObj_0000} \\
\multicolumn{3}{c}{Night Lens Flare} \\
\AddDetImgs{glare}{IMG_20210911_185558} \\
\multicolumn{3}{c}{Complex Lighting} \\
\AddDetImgs{incorrect_exposure}{2021-09-11-1146_8-CapObj_0000} \\
Lower 8 Bits of RAW Image & Higher 8 Bits of RAW Image & 8-bit RGB \\
\end{tabular}
\end{center}
\caption{\textbf{Visualizing the detection results under challenging light conditions for the RAW domain and RGB domain methods.}  The first column displays the lower 8 bits of the RAW data, which retains the shadow details often lost in standard RGB images due to brightness clipping. The second (middle) column presents the higher 8 bits of the RAW data, which contains the details in the bright areas. The third column uses the 8-bit RGB for detection. Detection results are overlaid for comparative study.}
%This side-by-side representation illustrate the enhanced dynamic range present in the single RAW image that the detection model input. The right column shows the processed 8-bit RGB images, providing a familiar point of comparison. {\it Zoom for better details.}}



\label{figure:r_detection_compare_visual}
\end{figure*}


==> sections/figures/r_detection_compare_visual_for_r1.tex <==
% \newcolumntype{M}[1]{>{\centering\arraybackslash}p{#1}}


% \newcommand{\AddDetImg}[2]{\includegraphics[width=#1\textwidth]{#2}}
% % 
% \newcommand{\AddDetImgs}[2]{
% \AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/ldr_raw.png} &
% \AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/hdr_raw.png} &
% \AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/rgb.png} \vspace{+6pt}
% }



\begin{figure*}
\begin{center}
% \begin{tabular}{p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ }}
\begin{tabular}{c@{ } c@{ } c@{ }}
\multicolumn{3}{c}{Facing the Sun} \\
\AddDetImgs{face_sun}{2021-09-11-0800_0-CapObj_0000} \\
\multicolumn{3}{c}{Night Lens Flare} \\
\AddDetImgs{glare}{IMG_20210911_185558} \\
\multicolumn{3}{c}{Complex Lighting} \\
\AddDetImgs{incorrect_exposure}{2021-09-11-1146_8-CapObj_0000} \\
Lower 8 Bits of RAW Image & Higher 8 Bits of RAW Image & Processed RGB \\
\end{tabular}
\end{center}
\caption{\textbf{Visualizing the detection results under challenging light conditions for the RAW domain and RGB domain methods.}  The first column displays the lower 8 bits of the RAW data, which retains the shadow details often lost in standard RGB images due to brightness clipping. The second (middle) column presents the higher 8 bits of the RAW data, which contains the details in the bright areas. The third column uses the RGB for detection. }

%\textbf{Visualizing RAW data for detection under challenging light conditions as compared to processed RGB images.} For the purpose of visualization, the left column displays the lower intensity values of the RAW data, which bring out shadow details often lost in standard RGB images due to brightness clipping. The middle column presents the higher intensity values of the RAW data, to emphasize details in the bright areas that typically get overlooked in processed images. This side-by-side representation serves to illustrate the enhanced dynamic range present in the single RAW image that the detection model input. The right column shows the processed 8-bit RGB images, providing a familiar point of comparison. {\it Zoom for better details.}}



\label{figure:r_detection_compare_visual_for_r_1}
\end{figure*}


==> sections/figures/r_detection_compare_visual_for_r2.tex <==
% \newcolumntype{M}[1]{>{\centering\arraybackslash}p{#1}}


% \newcommand{\AddDetImg}[2]{\includegraphics[width=#1\textwidth]{#2}}
% % 
% \newcommand{\AddDetImgs}[2]{
% \AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/ldr_raw.png} &
% \AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/hdr_raw.png} &
% \AddDetImg{0.28}{Figs/detection_visual_compare/#1/#2/rgb.png}
% }



\begin{figure*}
\begin{center}
% \begin{tabular}{p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ } p{0.155\textwidth}@{ }}
\begin{tabular}{c@{ } c@{ } c@{ }}
\multicolumn{3}{c}{Facing the Sun} \\
\AddDetImgs{face_sun}{2021-09-11-0800_0-CapObj_0000} \\
\multicolumn{3}{c}{Night Lens Flare} \\
\AddDetImgs{glare}{IMG_20210911_185558} \\
\multicolumn{3}{c}{Complex Lighting} \\
\AddDetImgs{incorrect_exposure}{2021-09-11-1146_8-CapObj_0000} \\
Lower 8 Bits of RAW Image & Higher 8 Bits of RAW Image & 8-bit RGB \\
\end{tabular}
\end{center}
\caption{\textbf{Visualizing the detection results under challenging light conditions for the RAW domain and RGB domain methods.}  The first column displays the lower 8 bits of the RAW data, which retains the shadow details often lost in standard RGB images due to brightness clipping. The second (middle) column presents the higher 8 bits of the RAW data, which contains the details in the bright areas. The third column uses the 8-bit RGB for detection.}
%This side-by-side representation illustrate the enhanced dynamic range present in the single RAW image that the detection model input. The right column shows the processed 8-bit RGB images, providing a familiar point of comparison. {\it Zoom for better details.}}



\label{figure:r_detection_compare_visual_for_r2}
\end{figure*}


==> sections/figures/r_hardware_results.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figs/pipeline_compare_results.pdf}
%\end{center}
\caption{{\bf Normalized Average Gains for $\rho$-Vision Compared to RGB-Vision.} Metrics are normalized to the results collected under the RGB-Vision framework, with the detection mAP tested using multiRAW (iPhone RAW). Latency refers to the total time consumption of the entire pipeline, power cost is measured using a power meter, and memory usage is monitored using an onboard tool (provided by the hardware platform).}
\label{fig:r_hardware_results}
\end{figure}


==> sections/figures/r_hardware_results_for_r2.tex <==
\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{Figs/pipeline_compare_results.pdf}
%\end{center}
\caption{{\bf Normalized Average Gains for $\rho$-Vision Compared to RGB-Vision.} Metrics are normalized to RGB-Vision framework evaluation results, with the mAP scores tested from multiRAW (iPhone RAW) detection tasks. Latency refers to the total time consumption of the entire pipeline, power cost is measured using a power meter, and memory usage is monitored during operation.}
\label{fig:r_hardware_results_for_r2}
\end{figure}


==> sections/figures/r_iem_ablation.tex <==
\begin{figure*}
    \centering
    
    \subfloat[simRAW is a superset of real RAW data]{\includegraphics[width=0.36\linewidth]{Figs/iem/plot.pdf} \label{fig:iem_plot}}
    \quad
    \subfloat[simRAW examples]{\includegraphics[width=0.593\linewidth]{Figs/iem/iem_visual.pdf} \label{fig:iem_visual}}

    
    \subfloat[ Testing RGB]{\includegraphics[width=0.19\linewidth]{Figs/iem/0000f77c-6257be58_small.png} \label{fig:bdd_sample}}
    \quad
    \subfloat[Random real RAW images from multiRAW dataset]{\includegraphics[width=0.77\linewidth]{Figs/iem/visual_batch_raw_small.png} \label{fig:iphone_batch_samples}}
    
    \subfloat[simRAW w/o IEM]{\includegraphics[width=0.19\linewidth]{Figs/iem/wo_iem_certain_small.png} \label{fig:wo_iem_certain}}
    \quad
    \subfloat[simulating RAW images by injecting noise to $E^{-1}(\cdot)$ outputs w/o using IEM]{\includegraphics[width=0.77\linewidth]{Figs/iem/wo_iem_random_small.png} \label{fig:wo_iem_random}}
    
    \caption{
    {\bf Evaluation of the Illumination Estimation Module (IEM). {\it Demosaicing has been applied to all images to enhance visibility.}} 
    (a) Adapting IEM to generate the simRAW's coverage using the mean color, where the color of each point $\phi_i$, $\theta_j$ represents the average color of a simRAW generated by sampled illumination parameters $\phi_i$, $\theta_j$. In contrast,  red markers indicate the average color of real RAW images.
    It clearly reveals that adapting IEM can cover all real-world illumination conditions in real RAW data. 
    (b)  simRAW examples generated by our Unpaired CycleR2R with various $\phi$, $\theta$, illustrating the IEM's ability to produce a wide range of illumination variations.
    (c) The corresponding RGB image fed into the invISP of our Unpaired CycleR2R, which is from the BDD100K dataset.
    (d) Random real RAW images from the multiRAW dataset, displaying the natural variability in illumination and color temperature.
    (e) Simulating a RAW image without using IEM can only produce a single simRAW per RGB input due to the absence of probabilistic illumination estimation. 
    (f) Simulating RAW images by injecting noise to $E^{-1}(\cdot)$ outputs, which can produce multiple simRAW samples without requiring IEM but demonstrate unrealistic diversity induction in RAW Images.  $E^{-1}(\cdot)$ is defined in invISP (see Fig. 2 in the main paper).
    }
    
    \label{fig:r_iem_ablation}
    \end{figure*}
    

==> sections/figures/segmentation.tex <==
% {\bf Segmentation Results}  Table~\ref{table:segmentation_results} presents segmentation results in the RAW and RGB domains for the six categories: road, traffic light, traffic sign, person, rider and car. The results show that the segmentation task in the RAW domain reduces latency with little loss (-1.3 mIOU) in segmentation performance. Figure~\ref{fig:detection_results} shows example results of our segmentation task in iRAW. We can see that the segmentation results of iRAW is very close to that of the RGB segmentation.

% \begin{table}[t]
% \begin{center}
% \caption{The FID \& MOS results of InvGamma~\cite{koskinen2019reverse}, CIE-XYZ Net~\cite{afifi2020cie}, CycleISP~\cite{zamir2020cycleisp} and our GAN-based invISP on BDD and D$^2$-City.}
% \begin{footnotesize}
% \begin{tabular}{c|c|c|cc}
% \hline
% \textbf{Metrics}                                    & \multicolumn{2}{c|}{\textbf{FID}$\downarrow$} & \multicolumn{2}{c}{\textbf{MOS$\uparrow$}}                  \\ \hline
% \textbf{Dataset}                                    & \textbf{BDD}    & \textbf{D$^2$-City}   & \multicolumn{1}{c|}{\textbf{BDD}} & \textbf{ D$^2$-City} \\ \hline
% \textbf{RGB}                                 & 155.69 & 197.98 & \multicolumn{1}{c|}{0.0} & 0.0 \\ \hline
% \textbf{InvGamma~\cite{koskinen2019reverse}} & 107.48          & 110.96          & \multicolumn{1}{c|}{1.1}             & 1.3              \\ \hline
% \textbf{CIE-XYZ Net~\cite{afifi2020cie}}              & 90.68  & 133.86 & \multicolumn{1}{c|}{2} & 2.6 \\ \hline
% \textbf{CycleISP~\cite{zamir2020cycleisp}}              & 93.09  & 106.28 & \multicolumn{1}{c|}{3.6} & 3.2 \\ \hline
% % \textbf{Our invISP framework without GAN}              & 95.40  & 108.56 & \multicolumn{1}{c|}{} &  \\ \hline
% \textbf{Our invISP}                          & \textbf{83.37}  & \textbf{92.56}  & \multicolumn{1}{c|}{\textbf{4}} & \textbf{4.1} \\ \hline
% \end{tabular}
% \label{table:fid_mos}
% \end{footnotesize}
% \end{center}
% \end{table}

\begin{comment}
\begin{table*}[t]
\begin{center}
\caption{Comparative studies of semantic segmentation in RGB domain and RAW domain.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|l|c}
\hline
\textbf{Domain} & \textbf{Road} & \textbf{Building} & \textbf{Fence} & \textbf{\begin{tabular}[c]{@{}c@{}}Traffic\\ Light\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Traffic\\ Sign\end{tabular}} & \textbf{Plant} & \textbf{Sky}   & \textbf{Person} & \textbf{Car}  & \textbf{Truck} & \textbf{Bus}   & \textbf{Bicycle} & \textbf{Delay} & \textbf{mIoU}  \\ \hline
\textbf{RGB}    & 96.45 & 94.65 & 90.62 & 54.34 & 87.91 & 94.89 & 99.03 & 49.88 & 88.70 & 94.00 & 92.51 & 64.77 & 36.7ms & \textbf{83.98} \\
\textbf{RAW}    & 96.13 & 94.15 & 90.34 & 53.75 & 86.44 & 94.61 & 98.76 & 49.93 & 88.33 & 93.60  & 87.49 & 64.14 & \textbf{6.4ms} & 83.14          \\ \hline
\end{tabular}%
}
\end{center}
\label{table:segmentation_results}
\end{table*}
\end{comment}

==> sections/figures/supp_hardware_results.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{Figs/pipeline_compare_results.pdf}
%\end{center}
\caption{{\bf Normalized Average Gains for $\rho$-Vision Compared to RGB-Vision.} Metrics are normalized to RGB-Vision framework evaluation results, with the mAP scores tested from multiRAW (iPhone RAW) detection tasks. Latency refers to the total time consumption of the entire pipeline, power cost is measured using a power meter, and memory usage is monitored during operation.}
\label{fig:supp_hardware_results}
\end{figure}


==> sections/tables/r_ablation_r2r.tex <==
\begin{table}
    \small
    \setlength{\tabcolsep}{5pt}
    \centering
    \caption{\textbf{Ablation of modular components of Unpaired CycleR2R}. KL divergence was assessed between real and simulated RAW images. Additionally, Recall and Average Precision (AP) metrics were evaluated using various RAW-domain detectors. These detectors were trained on simRAW images, generated by adapting modular settings in Unpaired CycleR2R, including BA and CC, AWB, and $\mathcal{L}_{var}$ }
    \label{table:r_ablation_r2r_component}
    \begin{tabular}{lcccccccc}
    \toprule
        \textbf{Method} & \textbf{AWB} & \textbf{BA} & \textbf{CC} & \textbf{IEM+$\mathcal{L}_{var}$} 
        & \textbf{KL} & \textbf{Recall} & \textbf{AP}    \\ \midrule
        InvGamma~\cite{koskinen2019reverse} 
        & - 
        & - 
        & - 
        & - 
        & 0.25
        & 68.6
        & 47.7
        \\ \midrule
        CycleISP~\cite{zamir2020cycleisp} 
        & - 
        & - 
        & - 
        & - 
        & 0.08
        & 71.6
        & 52.7
        \\ \midrule
        CIE-XYZ Net~\cite{afifi2020cie} 
        & - 
        & - 
        & - 
        & - 
        & 0.13
        & 72.2
        & 53.0
        \\ \midrule
        MBISPLD~\cite{conde2022model} 
        & - 
        & - 
        & - 
        & - 
        & 0.11
        & 73.0
        & 53.7
        \\ \midrule
        % \checkmark & & & & & 70.2 & 52.3\\ \midrule
        \multirow{4}{*}{Unpaired CycleR2R} 
        & \checkmark 
        & 
        & 
        & 
        & 0.12 
        & 71.9 
        & 53.6\\ 
        
        & \checkmark 
        & \checkmark 
        & 
        & 
        & 0.10
        & 72.5 
        & 54.9 \\  
        
        & \checkmark 
        & \checkmark 
        & \checkmark 
        & 
        & 0.09
        & 74.9 
        & 56.1 \\
        
        & \checkmark 
        & \checkmark 
        & \checkmark 
        & \checkmark 
        & \textbf{0.06} 
        & \textbf{76.1}  
        & \textbf{59.1} \\
    \bottomrule
    \end{tabular}
    \vspace{-8pt}
\end{table}


==> sections/tables/r_illumination.tex <==
\begin{table}[!h]
    \small
    \setlength{\tabcolsep}{3.5pt}
    \centering
    \caption{\textbf{Comparative analysis of object detection performance under different illumination conditions across object sizes.}}
    \label{r:ablation_illumination}
    
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Scenarios} &
    \textbf{Domain} & 
    $\textbf{mAP}_\text{small}$ &
    $\textbf{mAP}_\text{medium}$ &
    $\textbf{mAP}_\text{large}$ &
    \textbf{mAP} \\ \midrule
    \multirow{2}{*}{Day} 
    & RGB
    & 19.1
    & 54.9
    & 73.6
    & 58.5 \\
    
    & RAW
    & \textbf{21.2} 
    & \textbf{57.8}
    & \textbf{74.7}
    & \textbf{60.5} \\
    \midrule
    \multirow{2}{*}{Night} 
    & RGB 
    & 17.0
    & 49.1
    & 63.1
    & 56.1 \\

    & RAW
    & \textbf{28.2}
    & \textbf{54.5}
    & \textbf{67.7}
    & \textbf{59.8} \\
    \bottomrule
    \end{tabular}
    
\end{table}


==> sections/tables/r_training_data_compare.tex <==
\begin{table}[h]
    \centering
    \caption{\textbf{Performance Comparison of Unpaired CycleR2R with Different Inverse ISP Training Configurations}. Tests are evaluated on iPhone XSmax RAW. Training has two general configurations: the first uses BDD100K combined with iPhone RAW (denoted as ``b'' and ``i'', respectively), while the second employs a dataset formed by adjusting the white balance and exposure of RAW images from MultiRAW 7k, resulting in $\text{RGB}_\text{70k}$, in addition to the original $\text{RGB}_\text{7k}$. The ``Detector Train'' column indicates the dataset used in detector training, in which the terms ``b$\rightarrow$i'' and ``b$\rightarrow$7k'' represent conversion from BDD100K RGB image to the corresponding RAW sample by simulating iPhone RAW and MultiRAW 7k, respectively. }
    \label{tab:r_training_data_comparison}
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Unpaired CycleR2R} 
     &
     & \multicolumn{2}{c}{\textbf{Detector}} 

     & 
     & \multirow{2}{*}{\textbf{AP}} \\ \cmidrule{1-1} \cmidrule{3-4}
    Train
    &
    & Train
    & Test
    &
    & \\ \midrule
    $\text{RGB}_\text{b}$ + $\text{RAW}_\text{i}$ 
    &
    & $\text{simRAW}_\text{b$\rightarrow$i}$ 
    & $\text{RAW}_\text{i}$
    &
    & 59.1 \\ 
    $\text{RGB}_\text{7k}$ + $\text{RAW}_\text{7k}$ 
    &
    & $\text{simRAW}_\text{b$\rightarrow$7k}$ 
    & $\text{RAW}_\text{i}$
    &
    & 58.8 \\
    $\text{RGB}_\text{70k}$ + $\text{RAW}_\text{7k}$ 
    &
    & $\text{simRAW}_\text{b$\rightarrow$7k}$ 
    & $\text{RAW}_\text{i}$
    &
    & 58.7 \\ \bottomrule
    \end{tabular}
    \end{table}
    

==> sections/tables/r_unseen_camera.tex <==
\begin{table}[!h]
    \centering
    \caption{\textbf{Evaluation of Unpaired CycleR2R model on generalization to unseen camera data}: The model is trained on combinations of BDD100K RGB images and MultiRAW 7k RAW datasets, with one camera model omitted each time (notated as ``7k w/o x''). It is then tested on the RAW dataset of the excluded camera (``$\text{RAW}_\text{x}$'').  Average Precision (AP) scores are compared against that using the specific held-out camera's RAW images to train Unpaired CycleR2R  ($\text{RGB}_\text{b} + \text{RAW}_\text{x}$).}

    \label{tab:r_unseen_camera}
    \begin{tabular}{cccccc}
        \toprule
        \textbf{Unpaired CycleR2R} 
         &
         & \multicolumn{2}{c}{\textbf{Detector}} 
    
         & 
         & \multirow{2}{*}{\textbf{AP}} \\ \cmidrule{1-1} \cmidrule{3-4}
        Train
        &
        & Train
        & Test
        &
        & \\ \midrule
        $\text{RGB}_\text{b}$ + $\text{RAW}_\text{7k w/o i}$ 
        &
        & $\text{simRAW}_\text{b$\rightarrow$7k w/o i}$ 
        & $\text{RAW}_\text{i}$
        &
        & 58.5 \\ 
        $\text{RGB}_\text{b}$ + $\text{RAW}_\text{i}$ 
        &
        & $\text{simRAW}_\text{b$\rightarrow$i}$ 
        & $\text{RAW}_\text{i}$
        &
        & 59.1 \\ \midrule
        $\text{RGB}_\text{b}$ + $\text{RAW}_\text{7k w/o h}$ 
        &
        & $\text{simRAW}_\text{b$\rightarrow$7k w/o h}$ 
        & $\text{RAW}_\text{h}$
        &
        & 46.3 \\ 
        $\text{RGB}_\text{b}$ + $\text{RAW}_\text{h}$ 
        &
        & $\text{simRAW}_\text{b$\rightarrow$h}$ 
        & $\text{RAW}_\text{h}$
        &
        & 47.1 \\ \midrule
        $\text{RGB}_\text{b}$ + $\text{RAW}_\text{7k w/o a}$ 
        &
        & $\text{simRAW}_\text{b$\rightarrow$7k w/o a}$ 
        & $\text{RAW}_\text{a}$
        &
        & 50.5 \\ 
        $\text{RGB}_\text{b}$ + $\text{RAW}_\text{a}$ 
        &
        & $\text{simRAW}_\text{b$\rightarrow$a}$ 
        & $\text{RAW}_\text{a}$
        &
        & 51.7 \\ \bottomrule
    \end{tabular}
    \end{table}

==> sections/tables/r_without_labeled_detection.tex <==
\newcommand{\ie}{i.e.,}

\newcommand{\RGBcity}{$\text{RGB}_{\text{b}}$}
\newcommand{\RGBipone}{$\text{RGB}_{\text{i}}$}
% \newcommand{\RAWcity}{$\text{RAW}_{\text{b}}$}
\newcommand{\RAWipone}{$\text{RAW}_{\text{i}}$}
\newcommand{\pseudoRAWcity}{$\text{RAW}_{\text{b}}$}
\newcommand{\Baselines}{\textcolor{blue}{$\spadesuit$~}}
\newcommand{\InvISP}{\textcolor{orange}{$\blacksquare$~}}
\newcommand{\DomainAdap}{\textcolor{green}{$\blacklozenge$~}}
\newcommand{\Ours}{\textcolor{red}{$\bigstar$~}}

\begin{table*}
    \small
    \setlength{\tabcolsep}{6pt}
    \centering
    \caption{
    {\textbf{Recall and Average Precision (AP) of Object Detection on the testing set of iPhone RAWs.} RGB detector is trained using original RGB images in \textit{BDD100K}~\cite{yu2020bdd100k} (e.g., \RGBcity); Various simRAW datasets associated with \RGBcity~are generated using different methods which are simply marked as sim\pseudoRAWcity~to train the RAW detector. 
    The testing RAW images in iPhone RAW \RAWipone~and their paired RGB images in \RGBipone~converted using built-in iPhone ISP are tested accordingly.
    All detectors are shared with the same head, \ie, YOLOv3~\cite{yolo} and the same backbone, \ie, MobileNetV2~\cite{sandler2018mobilenetv2} for a fair comparison.
    \Baselines Baselines, \DomainAdap Domain Adaptation Solutions, \InvISP invISP Methods, \Ours Ours.}
    }
    \label{table:r_without_labeled_detection}
    \begin{tabular}{lrrrrr}
    \toprule
            \textbf{Method} & \textbf{ invISP Training} & \textbf{Detector Training} & \textbf{Detector Testing} & \textbf{Recall} & \textbf{AP}    \\ \midrule
         \Baselines Naive Baseline & -  & \RGBcity & \RAWipone & 67.5 & 51.1 \\ 
         \Baselines RGB Baseline  & -  & \RGBcity & \RGBipone & 74.7 & 55.6 \\ \midrule
        % \DomainAdap CycleGAN (ICCV'17)~\cite{zhu2017unpaired} &  -  &  \RGBcity,~\RAWipone & \RAWipone  & 10.8 & 3.9 \\
        \DomainAdap DA-Faster (CVPR'18)~\cite{chen2018domain} &  -  &  \RGBcity,~\RAWipone & \RAWipone  & 13.7 & 12.9 \\
        \DomainAdap MS-DAYOLO (ICIP'21)~\cite{hnewa2021multiscale} &  -  & \RGBcity,~\RAWipone & \RAWipone  & 31.2 & 29.7 \\
        \DomainAdap AT (CVPR'22)~\cite{li2022cross} &  -  & \RGBcity,~\RAWipone & \RAWipone  & 68.9 & 53.2 \\\midrule
        \InvISP InvGamma (ICIP'19)~\cite{koskinen2019reverse} &  \RGBipone,~\RAWipone  & sim\pseudoRAWcity & \RAWipone  & 68.6 & 48.7 \\
        \InvISP CycleISP (CVPR'20)~\cite{zamir2020cycleisp} & \RGBipone,~\RAWipone  & sim\pseudoRAWcity & \RAWipone & 71.6 & 52.7 \\ 
        % \InvISP Invertible-ISP (CVPR'21)~\cite{xing2021invertible} & \RGBipone,~\RAWipone & \pseudoRAWcity & \RAWipone & - & - \\ 
        \InvISP CIE-XYZ Net (TPAMI'21)~\cite{afifi2020cie} & \RGBipone,~\RAWipone & sim\pseudoRAWcity & \RAWipone & 72.2 & 53.0 \\ 
        % % Marcos~\cite{conde2022model} & simu RAW & RAW & 0.091 & 0.010 \\ \midrule
        \InvISP MBISPLD (AAAI'22)~\cite{conde2022model} & \RGBipone,~\RAWipone & sim\pseudoRAWcity & \RAWipone & 73.0 & 53.7 \\ \midrule
        \Ours \textbf{Unpaired CycleR2R} & \RGBcity,~\RAWipone & sim\pseudoRAWcity & \RAWipone & \textbf{76.1}  & \textbf{59.1} \\
    \bottomrule
    \end{tabular}
\end{table*}


==> sections/tables/r_without_labeled_detection_for_r1.tex <==
% \newcommand{\ie}{i.e.,}

% \newcommand{\RGBcity}{$\text{RGB}_{\text{b}}$}
% \newcommand{\RGBipone}{$\text{RGB}_{\text{i}}$}
% % \newcommand{\RAWcity}{$\text{RAW}_{\text{b}}$}
% \newcommand{\RAWipone}{$\text{RAW}_{\text{i}}$}
% \newcommand{\pseudoRAWcity}{$\text{RAW}_{\text{b}}$}
% \newcommand{\Baselines}{\textcolor{blue}{$\spadesuit$~}}
% \newcommand{\InvISP}{\textcolor{orange}{$\blacksquare$~}}
% \newcommand{\DomainAdap}{\textcolor{green}{$\blacklozenge$~}}
% \newcommand{\Ours}{\textcolor{red}{$\bigstar$~}}

\begin{table*}
    \small
    \setlength{\tabcolsep}{6pt}
    \centering
    \caption{
    {\textbf{Recall and Average Precision (AP) of Object Detection on the testing set of iPhone RAWs.} RGB detector is trained using original RGB images in \textit{BDD100K}~\cite{yu2020bdd100k} (e.g., \RGBcity); Various simRAW datasets associated with \RGBcity~are generated using different methods which are simply marked as sim\pseudoRAWcity~to train the RAW detector. 
    The testing RAW images in iPhone RAW \RAWipone~and their paired RGB images in \RGBipone~converted using built-in iPhone ISP are tested accordingly.
    All detectors are shared with the same head, \ie, YOLOv3~\cite{yolo} and the same backbone, \ie, MobileNetV2~\cite{sandler2018mobilenetv2} for a fair comparison.
    \Baselines Baselines, \DomainAdap Domain Adaptation Solutions, \InvISP invISP Methods, \Ours Ours.}
    }
    \label{table:r_without_labeled_detection_for_r1}
    \begin{tabular}{lrrrrr}
    \toprule
            \textbf{Method} & \textbf{ invISP Training} & \textbf{Detector Training} & \textbf{Detector Testing} & \textbf{Recall} & \textbf{AP}    \\ \midrule
         \Baselines Naive Baseline & -  & \RGBcity & \RAWipone & 67.5 & 51.1 \\ 
         \Baselines RGB Baseline  & -  & \RGBcity & \RGBipone & 74.7 & 55.6 \\ \midrule
        % \DomainAdap CycleGAN (ICCV'17)~\cite{zhu2017unpaired} &  -  &  \RGBcity,~\RAWipone & \RAWipone  & 10.8 & 3.9 \\
        \DomainAdap DA-Faster (CVPR'18)~\cite{chen2018domain} &  -  &  \RGBcity,~\RAWipone & \RAWipone  & 13.7 & 12.9 \\
        \DomainAdap MS-DAYOLO (ICIP'21)~\cite{hnewa2021multiscale} &  -  & \RGBcity,~\RAWipone & \RAWipone  & 31.2 & 29.7 \\
        \DomainAdap AT (CVPR'22)~\cite{li2022cross} &  -  & \RGBcity,~\RAWipone & \RAWipone  & 68.9 & 53.2 \\\midrule
        \InvISP InvGamma (ICIP'19)~\cite{koskinen2019reverse} &  \RGBipone,~\RAWipone  & sim\pseudoRAWcity & \RAWipone  & 68.6 & 48.7 \\
        \InvISP CycleISP (CVPR'20)~\cite{zamir2020cycleisp} & \RGBipone,~\RAWipone  & sim\pseudoRAWcity & \RAWipone & 71.6 & 52.7 \\ 
        % \InvISP Invertible-ISP (CVPR'21)~\cite{xing2021invertible} & \RGBipone,~\RAWipone & \pseudoRAWcity & \RAWipone & - & - \\ 
        \InvISP CIE-XYZ Net (TPAMI'21)~\cite{afifi2020cie} & \RGBipone,~\RAWipone & sim\pseudoRAWcity & \RAWipone & 72.2 & 53.0 \\ 
        % % Marcos~\cite{conde2022model} & simu RAW & RAW & 0.091 & 0.010 \\ \midrule
        \InvISP MBISPLD (AAAI'22)~\cite{conde2022model} & \RGBipone,~\RAWipone & sim\pseudoRAWcity & \RAWipone & 73.0 & 53.7 \\ \midrule
        \Ours \textbf{Unpaired CycleR2R} & \RGBcity,~\RAWipone & sim\pseudoRAWcity & \RAWipone & \textbf{76.1}  & \textbf{59.1} \\
    \bottomrule
    \end{tabular}
\end{table*}


==> sections/tables/r_wo_labeled_classification.tex <==
\newcommand{\RGBImageNet}{$\text{RGB}_{\text{IN}}$}
\newcommand{\RGBpixel}{$\text{RGB}_{\text{AX}}$}
\newcommand{\RGBpixelpixel}{$\text{RGB}_{\text{GP}}$}
\newcommand{\RGBpixelAI}{$\text{RGB}_{\text{AX-AI}}$}
\newcommand{\RAWpixel}{$\text{RAW}_{\text{GP}}$}
\newcommand{\pseudoRAWpixel}{$\text{RAW}_{\text{IN}}$}
\newcommand{\RGBanscombe}{$\text{RGB}_{\text{Ans-ISP}}$}
% \newcommand{\RAWcity}{$\text{RAW}_{\text{b}}$}
% \newcommand{\RAWipone}{$\text{RAW}_{\text{i}}$}
% \newcommand{\pseudoRAWcity}{$\text{RAW}_{\text{c}}$}
% \newcommand{\Baselines}{\textcolor{blue}{$\spadesuit$~}}
% \newcommand{\InvISP}{\textcolor{orange}{$\blacksquare$~}}
% \newcommand{\DomainAdap}{\textcolor{green}{$\blacklozenge$~}}
% \newcommand{\Ours}{\textcolor{red}{$\bigstar$~}}
% \newcommand{\RGBipone}{$\text{RGB}_{\text{i}}$}
% \newcommand{\RGBanscombe}{$\text{RGB}_{\text{Ans-ISP}}$}
% \newcommand{\RAWcity}{$\text{RAW}_{\text{b}}$}
% \newcommand{\RAWipone}{$\text{RAW}_{\text{i}}$}
% \newcommand{\pseudoRAWcity}{$\text{RAW}_{\text{c}}$}
% \newcommand{\Baselines}{\textcolor{blue}{$\spadesuit$~}}
% \newcommand{\InvISP}{\textcolor{orange}{$\blacksquare$~}}
% \newcommand{\DomainAdap}{\textcolor{green}{$\blacklozenge$~}}
% \newcommand{\Ours}{\textcolor{red}{$\bigstar$~}}

\begin{table*}[!h]
    \small
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{
    {\textbf{Classification Accuracy On Google Pixel RAW images.}
    %Classifier training was performed on RGB images from the ImageNet dataset (\RGBImageNet) and simulated RAW Pixel images (sim\pseudoRAWpixel), using the simple Mosaic or Unpaired CycleR2R method for synthesis. The evaluation involved testing the classifiers on \RAWpixel~ images after being processed by the respective inverse ISP techniques. The table reports Top-1 and Top-5 accuracy metrics, the number of parameters (\# Parameters), and the computational complexity in terms of FLOPs (Floating Point Operations).
    }
    }
    \label{table:r_wo_labeled_classification}
    
    \begin{threeparttable}
    \begin{tabular}{lcrcccccccccc}
    \toprule
            \multirow{2}*{\textbf{Method}}
            & \textbf{invISP}
            &
            & \multicolumn{2}{c}{\textbf{Classifier}}
            &
            & \multirow{2}*{\textbf{Top-1 Acc.}}
            & \multirow{2}*{\textbf{Top-5 Acc.}}
            & \multirow{2}*{\textbf{\# Parameters}}
            & \multirow{2}*{\textbf{FLOPs}}
            \\\cmidrule{2-2}\cmidrule{4-5}
            
            & {\textbf{Train}}
            &
            & {\textbf{Train}}
            & {\textbf{Test}}
            &
            &
            &
            & 
            &
            \\ \midrule
         Anscombe ISP\tnote{*}~\cite{diamond2021dirty} 
        & -
        &
        &  \RGBanscombe
        & \RGBanscombe
        &  
        & 33.1
        & 58.4
        & 4.28
        & 282
        \\
        Mosaic RAW\tnote{*}~\cite{diamond2021dirty} 
        & -
        &
        & sim\pseudoRAWpixel
        & \RAWpixel        
        &  
        & 27.0
        & 52.5
        & \textbf{4.23}
        & \textbf{181}
        \\ \midrule
        \textbf{Unpaired CycleR2R} 
        & \RGBImageNet,~\RAWpixel
        &
        & sim\pseudoRAWpixel
        & \RAWpixel  
        &  
        & \textbf{35.5}
        & \textbf{72.1}
        & \textbf{4.23}
        & \textbf{181}
        \\
    \bottomrule
    \end{tabular}
    
    \begin{tablenotes}
        \item[*] Both the Anscombe ISP and Mosaic RAW apply simple mosaic operations to generate RAW samples from the corresponding RGB images. They don't need to train the invISP. 
    \end{tablenotes}
    % \vspace{2mm}
    % Such a mosaic operation is  referred to~\cite{}
\end{threeparttable}
\end{table*}


==> sections/tables/supp_ablation_gamma.tex <==
\begin{table*}
    \small
    \setlength{\tabcolsep}{5.5pt}
    \centering
    \caption{Impact of Gamma Correction (GC) on segmentation.}
    \label{table:supp_ablation_gamma}
    \begin{threeparttable}
    \begin{tabular}{lccccccccccccc}
    \toprule
    \textbf{Domain} & 
    \textbf{Road} &
    \textbf{Building} &
    \textbf{Fence} &
    \textbf{Tr. Light} &
    \textbf{Tr. Sign} &
    \textbf{Plant} &
    \textbf{Sky} &
    \textbf{Person} &
    \textbf{Car} &
    \textbf{Truck} &
    \textbf{Bus} &
    \textbf{Bicycle} &
    \textbf{mIoU} \\ \midrule
    RGB &
    \textbf{91.7} &
    81.6 &
    \textbf{56.4} &
    39.2 &
    \textbf{73.5} &
    \textbf{92.2} &
    95.1 &
    \textbf{34.3} &
    \textbf{66.3} &
    \textbf{55.8} &
    \textbf{68.7} &
    \textbf{47.2} &
    \textbf{66.8} \\
    RAW w/o GC &
    35.8 &
    44.2 &
    20.0 &
    9.7 &
    14.8 &
    42.4 &
    95.8 &
    14.4 &
    20.9 &
    9.1 &
    35.7 &
    12.7 &
    29.6 \\
    RAW w/ GC &
    89.3 &
    \textbf{83.2} &
    56.1 &
    \textbf{40.2} &
    70.9 &
    91.2 &
    \textbf{96.9} &
    34.0 &
    65.8 &
    48.1 &
    63.6 &
    41.4 &
    65.0 \\
    \bottomrule
    \end{tabular}
    
    \begin{tablenotes}
        \footnotesize 
        \item \textbf{Tr. Light} $\leftarrow$ Traffic Light; \textbf{Tr. Sign} $\leftarrow$ Traffic Sign.
    \end{tablenotes}
    
    \end{threeparttable}
    
\end{table*}




==> supp_material_aux.tex <==


